VC Classes are Adversarially Robustly Learnable, but Only Improperly

We study the question of learning an adversarially robust predictor. We show that any hypothesis class $\mathcal{H}$ with finite VC dimension is robustly PAC learnable with an improper learning rule. The requirement of being improper is necessary as we exhibit examples of hypothesis classes $\mathcal{H}$ with finite VC dimension that are not robustly PAC learnable with any proper learning rule.

==> related-work.tex <==
\section{Related Work}
\label{sec:relatedwork}
% Work that considers proper learning algorithms
\paragraph{Robust Generalization} A standard approach to establish robust generalization guarantees for RERM and proper learning algorithms is through uniform convergence (citations?). This requires studying and analyzing the complexity of the robust loss class which is the approach taken in a few recent works \citep{bubeck2018adversarial,cullina2018pac,khim2018adversarial,yin2018rademacher,attias2018improved}. \citet{bubeck2018adversarial} showed that for continuous distributions that admit robust classifiers, the sample complexity of RERM is bounded by the log of a robust notion of covering number. \citet{cullina2018pac} showed that the sample complexity of RERM in the worst case is upperbounded by the VC-dimension of the robust loss class. They showed that for linear classifiers and $(\ell_p,p\geq 1)$ norm-bounded adversaries, the VC dimension of the robust loss class $\vc(\L_{\H}^{\U})$ is equal to the VC dimension of linear classifiers $\vc(\H)$. \citet{khim2018adversarial,yin2018rademacher} studied the Rademacher complexity of the robust loss class for linear classifiers and feedforward neural networks, where they bound the sample complexity of RERM with respect to surrogate losses (e.g.\ hinge loss and cross-entropy loss).

\citet{attias2018improved} considered classes of adversaries $\U$ where $|\U(x)|\leq k$, i.e.\ for each input example the number number of adversarial perturbations is bounded by $k$. They showed that any hypothesis class $\H$ with finite VC dimension can be robustly learned with a sample complexity of $\O\left(\frac{1}{\eps^2}((k\log k)\vc{(\H)}+\log1/\delta)\right)$. Although the algorithm proposed is \emph{improper}, we note that $\RERM$ also works in this setup, because their analysis is based on uniform convergence. As a consequence of our work, we find that the dependence on $k$ can be improved to $O(\log k)$ (see Section 5). 

% Bubeck et al. The main result of the paper is a classification task where it is easy to learn non-robustly but computationally intractable to learn robustly in the Statistical Query model.
% Bubeck showed that for finite hypothesis classes $\H$, the sample complexity of RERM is bounded by $\log|\H|$ (this is an upperbound on the VC-dimension of the robust loss class).

\citet{schmidt2018adversarially} showed that there exists a family of distributions (mixtures of two $d$-dimensional spherical Gaussians) where the sample complexity for standard learning is $O(1)$, but the sample complexity to robustly learn against $\ell_\infty$ perturbations of magnitude $\gamma$ is at least $\Omega(\frac{\gamma^2\sqrt{d}}{\log d})$. This an interesting instance where there is a large separation in sample complexity between standard learning and adversarially robust learning. In this paper, we are interested in studying the sample complexity of adversarially robust learning in a distribution-free setting.

\citet{1710.10571,lee2018minimax} consider a more general framework of robust learning, usually referred to as distributional robustness, where the goal is to minimize the worst-case loss with respect to distributions that are close to the original data distribution under the Wasserstein metric. They propose learning algorithms with robust generalization guarantees but only for smooth or Lipschitz loss functions (which doesn't include the robust $0$-$1$ loss studied in this paper). The sample complexity is controlled by the covering number of the loss function class.

\citet{xu2012robustness} established that a certain notion of algorithmic robustness implies generalization in the standard $0$-$1$ loss learning setting. In contrast, our work is concerned with establishing generalization guarantees in the robust $0$-$1$ loss learning setting.

%mention work on robust optimization?
\paragraph{Robust Empirical Risk Minimization}There is a lot of work focusing on designing algorithms to solve the robust empirical risk minimization (RERM) problem. The class of adversaries $\U$ that is typically considered is norm-bounded adversaries. For binary linear classifiers, \citep{xu2009robustness} established that RERM with respect to the hinge loss and Soft-margin SVMs are equivalent optimization problems. More recently there has been a lot of work on training adversarially robust deep neural networks. \citet{madry2017towards} proposed solving the RERM problem using first-order methods. \citet{wong2018provable, raghunathan2018certified, raghunathan2018semidefinite} use first-order methods to minimize surrogate adversarial losses that are tight upperbounds of the original adversarial loss. They provide efficiently computable certificates that upperbound the robust test accuracy which is useful in practice. When viewed as learning algorithms, we note that all of these approaches are categorized as proper learning algorithms where their robust generalization guarantees are not well-understood. One of the main results in this paper suggests that the large gap that is empirically observed between robust train accuracy and robust test accuracy could be because proper learning algorithms are being used. There is also a whole family of different non-certified algorithms for training robust neural networks. These algorithms are usually broken (their robust test accuracy is driven to zero) not long after they are announced \citep{athalye2018obfuscated}.

% can improve upone this with $\log k vc(H) O(1/\eps)$. they could have done proper learning
% proper learning is enough in this. 


% considering such work, why is our work important? we could say that if Rademacher doesn't blow up too much, based on what these papers say, then we should expect these robust minimizers to generalize well, but that is not what is observed in practice.

% Work on the generalization part of the problem
%It was empirically observed in \citep{schmidt2018adversarially} that training deep learning models to be robust against first-order adversaries by minimizing the adversarial loss does not actually guarantee that the model will generalize robustly. For example, training a Resnet model on CIFAR10 with the PGD adversarial training algorithm yields a model with adversarial training accuracy of $96\%$ and adversarial test accuracy of only $47\%$. 

%\citet{schmidt2018adversarially} established that the sample complexity to robustly classify two $d$-dimensional spherical Gaussians (where the means are $2\sqrt{d}$ apart) with $\ell_{\infty}$ perturbations of at most $\gamma$ is lower bounded by $\Omega(\frac{\gamma^2\sqrt{d}}{\log d})$. They also showed that there is a proper learning algorithm with respect to the class of halfspaces that can achieve robust error at most 1\% with sample complexity $O(\gamma^2\sqrt d)$. We remark here that this result does not imply that the sample complexity to agnostically $\gamma$-robustly PAC learn halfspaces is strictly higher than the VC-dimension $d$. 


==> review-response.tex <==
We thank the reviewer for the helpful comments and valuable feedback. We will work on adding more clarifying details in section 4 and shorten the presentation of section 3.

Reviewer 1:

We also wanted to note that the result in Lemma 2 holds when U(x) is a ball with radius gamma around x with respect to some metric. Even in this case, which is relevant in practice, we get a large blow up in the VC dimension of the robust loss function. 

Reviewer 2:

We agree that presenting the main theorem in section 4 in terms of vc(H) and vc*(H) would more precise. We can also probably mention example of hypothesis classes H where vc*(H) is polynomial in vc(H).

For an arbitrary adversary U, one can view realizable robust PAC learning of a class H as a special case that considers only distributions D that admit a robust classifier h in H. We argue that this is meaningful to study, because one can think of real-world scenarios where there is a notion of "margin" between objects corresponding to different classes. 

For example, when U(x) a ball with radius gamma around x with respect to Euclidean distance, and H is the set of halfspaces, it is easy to see that robust PAC learning in this case is equivalent to learning with a margin condition. So, in a sense, realizable robust PAC learning seems to be "easier" in terms of sample complexity. 

Lemma 3 also holds for randomized learning rules.

Regarding comparing our work to Feige, Mansour, and Schapire (2015), in section 4, we provide a detailed comparison with a more resent work by Attias, Kontorovich, and Mansour (2018) that extends upon the results of that previous work (see remark on related work).

Reviewer 3:

While it is true that there will be many situations where the robust loss (and RERM) can't be efficiently computed, this paper studies the sample complexity of robust PAC learning and does not consider the computational aspects of the problem. However, in the fourth paragraph of the discussion section, we discuss in detail open questions that are related to the computational aspects of robust PAC learning.

In the proof of Lemma 2, we choose to not include the original sample in the union (i.e. all predictors will label it with +1), because it simplifies the proof of Theorem 1.

